Anomaly Detection Framework Using Rule Extraction for Efficient Intrusion Detection

Huge datasets in cyber security, such as network traffic logs, can be analyzed using machine learning and data mining methods. However, the amount of collected data is increasing, which makes analysis more difficult. Many machine learning methods have not been designed for big datasets, and consequently are slow and difficult to understand. We address the issue of efficient network traffic classification by creating an intrusion detection framework that applies dimensionality reduction and conjunctive rule extraction. The system can perform unsupervised anomaly detection and use this information to create conjunctive rules that classify huge amounts of traffic in real time. We test the implemented system with the widely used KDD Cup 99 dataset and real-world network logs to confirm that the performance is satisfactory. This system is transparent and does not work like a black box, making it intuitive for domain experts, such as network administrators.

==> Makefile <==
NAME=ids_dm_cre_elsevier

# The files that are required in Elsevier journal submission:
SRCFILES = ids_dm_cre_elsevier.tex abstract.tex conclusion.tex \
	ids_dm_cre_elsevier.bbl ids_dm_cre.bib \
	introduction.tex method.tex related.tex results_iris.tex \
	results_kdd.tex results_log.tex \
	pics/Fig1.pdf \
	pics/Fig2.pdf \
	pics/Fig3.pdf \
	pics/Fig4.pdf \
	pics/Fig5.pdf \
	pics/Fig6.pdf \
	pics/Fig7.pdf \
	pics/Fig8.pdf \
	pics/Fig9.pdf \
	pics/Fig10.pdf \
	pics/Fig11.pdf \
	pics/Fig12.pdf \
	tables/10_5000_5000_accuracy.tex tables/10_5000_5000_cm.tex \
	tables/10_whole_accuracy.tex tables/10_whole_cm.tex \
	tables/log_100_train.tex tables/log_500_train.tex tables/model_cm.tex \
	algorithm2e.sty numcompress.sty \
	elsarticle.cls model4-names.bst \
	Makefile 

all: elsevier

.PHONY: pics
pics:
	export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
	cd pics; for f in *.eps; do epstopdf $$f; done	

pdf:
	pdflatex ${NAME}
	bibtex ${NAME}
	pdflatex ${NAME}
	pdflatex ${NAME}

# Journal version for Springer:
springer: pdf
	pdflatex $(NAME)
	pdflatex $(NAME)
	pdflatex $(NAME)

# Journal version for Elsevier:
elsevier: pdf
	pdflatex $(NAME)
	pdflatex $(NAME)
	pdflatex $(NAME)

final: pdf
	pdf2ps ${NAME}.pdf tmp.ps
	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true tmp.ps ${NAME}_final.pdf
	rm tmp.ps

$(NAME)_springer.bbl:
	pdflatex $(NAME)_springer
	bibtex $(NAME)

$(NAME)_elsevier.bbl:
	pdflatex $(NAME)_elsevier
	bibtex $(NAME)

# Source package:
# If needed, we could substitute the bibliography generation here.
package: $(SRCFILES)
	mkdir ids_dm_cre_sources
	cp $(SRCFILES) ids_dm_cre_sources
	sed -i 's/tables\///g' ids_dm_cre_sources/results_kdd.tex
	sed -i 's/tables\///g' ids_dm_cre_sources/results_log.tex
	sed -i 's/tables\///g' ids_dm_cre_sources/method.tex
	sed -i 's/tables\///g' ids_dm_cre_sources/method.tex
	echo "ARE YOU AN WIZARD?"
	-rm ids_dm_cre_sources.zip
	zip -r ids_dm_cre_sources.zip ids_dm_cre_sources

clean:
	-rm *.aux
	-rm *.log
	-rm *.bbl
	-rm *.blg
	-rm *.spl
	-rm *.fff
	-rm *.ttt
	-rm *.lof
	-rm *.lot
	-rm -r ids_dm_cre_sources

